The angular power spectrum measurement of the Galactic synchrotron emission in two fields of the TGSS survey

Characterizing the diffuse Galactic synchrotron emission at arcminute angular scales is needed to reliably remove foregrounds in cosmological 21-cm measurements. The study of this emission is also interesting in its own right. Here, we quantify the fluctuations of the diffuse Galactic synchrotron emission using visibility data for two of the fields observed by the TIFR GMRT Sky Survey (TGSS). We have used the 2D Tapered Gridded Estimator (TGE) to estimate the angular power spectrum $(C_{\ell})$ from the visibilities. We find that the sky signal, after subtracting the point sources, is likely dominated by the diffuse Galactic synchrotron radiation across the angular multipole range $240 \le \ell \lesssim 500$. We present a power law fit, $C_{\ell}=A\times\big(\frac{1000}{l}\big)^{\beta}$, to the measured $C_{\ell}$ over this $\ell$ range. We find that $(A,\beta)$ have values $(356\pm109~{\rm mK^2},2.8\pm0.3)$ and $(54\pm26~{\rm mK^2},2.2\pm0.4)$ in the two fields. For the second field, however, there is indication of a significant residual point source contribution, and for this field we interpret the measured $C_{\ell}$ as an upper limit for the diffuse Galactic synchrotron emission. While in both fields the slopes are consistent with earlier measurements, the second field appears to have an amplitude which is considerably smaller compared to similar measurements in other parts of the sky.

==> readme <==
%auto-ignore

This file contain information regarding the paper "The angular power spectrum measurement of the Galactic synchrotron emission in two  fields of the TGSS survey"

Authors:Samir Choudhuri, Somnath Bharadwaj, Sk. Saiyad Ali, Nirupam Roy ,H.T. Intema, and Abhik Ghosh

Comments: 6 pages, 1 table, 3 figures, Accepted for publication in MNRAS Letters. The definitive version will be available at http://mnrasl.oxfordjournals.org/

The contact details of the first author are as follows
Samir Choudhuri
email  : samir11@phy.iitkgp.ernet.in
Address: Indian Institute of Technology Kharagpur
         Kharagpur-721302, India



Abstract:Characterizing the diffuse Galactic synchrotron emission at arcminute angular scales is needed to reliably remove foregrounds in
cosmological 21-cm measurements. The study of this emission is also
interesting in its own right. Here, we quantify the fluctuations of
the diffuse Galactic synchrotron emission using visibility data for
two of the fields observed by the TIFR GMRT Sky Survey (TGSS).  We have
used the 2D Tapered Gridded Estimator (TGE) to estimate the angular
power spectrum $(C_{\ell})$ from the visibilities. We find that the
sky signal, after subtracting the point sources, is likely
dominated by the diffuse Galactic synchrotron radiation across the angular multipole range $240 \le \ell \lesssim 500$. 
 We present a power law fit, $C_{\ell}=A\times\big(\frac{1000}{l}\big)^{\beta}$, to the measured $C_{\ell}$ over this $\ell$ range. We find that $(A,\beta)$ have values $(356\pm109~{\rm mK^2},2.8\pm0.3)$ and 
$(54\pm26~{\rm mK^2},2.2\pm0.4)$ in the two fields. For the second field, however,   there is indication of a significant residual point source contribution, and for this field we interpret the measured $C_{\ell}$ as an upper limit for the  diffuse Galactic synchrotron emission. While in both fields the slopes are consistent with earlier measurements, the second field appears to have an amplitude which is considerably smaller compared to similar measurements  in other parts of the sky.


The compressed tar file "TGE_TGSS_arxiv.tar.gz" contain the following files:

readme : This file
ms.tex : Manuscript file in LaTeX format
mn2e.cls : Manuscript class file
fig1.ps: (Fig 1 left panel)
fig4.ps: (Fig 1 right panel)
fig2.ps: (Fig 2)
fig3.ps: (Fig 3 left panel)
fig6.ps: (Fig 3 right panel)

